Multi-Scale Stellar Associations across the Star Formation Hierarchy in PHANGS-HST Nearby Galaxies: Methodology and Properties

We develop a method to identify and determine the physical properties of stellar associations using Hubble Space Telescope (HST) NUV-U-B-V-I imaging of nearby galaxies from the PHANGS-HST survey. We apply a watershed algorithm to density maps constructed from point source catalogues Gaussian smoothed to multiple physical scales from 8 to 64 pc. We develop our method on two galaxies that span the distance range in the PHANGS-HST sample: NGC 3351 (10 Mpc), NGC 1566 (18 Mpc). We test our algorithm with different parameters such as the choice of detection band for the point source catalogue (NUV or V), source density image filtering methods, and absolute magnitude limits. We characterise the properties of the resulting multi-scale associations, including sizes, number of tracer stars, number of associations, photometry, as well as ages, masses, and reddening from Spectral Energy Distribution fitting. Our method successfully identifies structures that occupy loci in the UBVI colour-colour diagram consistent with previously published catalogues of clusters and associations. The median ages of the associations increases from log(age/yr) = 6.6 to log(age/yr) = 6.9 as the spatial scale increases from 8 pc to 64 pc for both galaxies. We find that the youngest stellar associations, with ages < 3 Myr, indeed closely trace H ii regions in H$\alpha$ imaging, and that older associations are increasingly anti-correlated with the H$\alpha$ emission. Owing to our new method, the PHANGS-HST multi-scale associations provide a far more complete census of recent star formation activity than found with previous cluster and compact association catalogues. The method presented here will be applied to the full sample of 38 PHANGS-HST galaxies.

==> PHANGS-HST_ Stellar Associations ( For submission) (ArXiv)/lowRes_figs/00notes.tex <==
Brad, I think this is a important point, and I agree that it could be an issue.  Right now the only way that it is addressed is by imposing a lower limit on the masses of the associations that are included.  We might also only overlay the higher mass young associations with the CO.  There’s definitely a lot of CO in optically dark regions though, and in those cases there wouldn’t be any Halpha emission overlapping the CO. I’ll put this in the to-do list for new overleaf for the second paper to remind us to look at it.  -Janice
 
From: Brad Whitmore <whitmore@stsci.edu>
Date: Monday, October 26, 2020 at 10:07 AM
To: Kirsten Larson <kllarson@gmail.com>
Cc: Brad Whitmore <whitmore@stsci.edu>, Janice Lee <janice@ipac.caltech.edu>
Subject: 10 brightest and 10 faintest, < 5 myr clusters relative to the CO clouds in the disk regions.
 
Hi Kristen – I am still worried that we may be degrading the correlation between positions of associations and CO peaks by including  low S/N objects. Could you show an image and plot (for both 3351 and 1556) with ONLY the 10 brightest < 5 myr clusters relative to the CO clouds in the disk region.
 
Then try the same things for the 10 faintest (expect this one to be pretty random)
 
Then do the same for the oldest associations (expect these to be pretty random)
 
Sorry to keep pushing this but I am use to seeing the youngest, brightest clusters right on top of the Halpha, and since Halpha correlates well with CO, I expect the them to be right on top of the CO.
 
Cheers,
Brad

==> lowRes_figs/00notes.tex <==
Brad, I think this is a important point, and I agree that it could be an issue.  Right now the only way that it is addressed is by imposing a lower limit on the masses of the associations that are included.  We might also only overlay the higher mass young associations with the CO.  There’s definitely a lot of CO in optically dark regions though, and in those cases there wouldn’t be any Halpha emission overlapping the CO. I’ll put this in the to-do list for new overleaf for the second paper to remind us to look at it.  -Janice
 
From: Brad Whitmore <whitmore@stsci.edu>
Date: Monday, October 26, 2020 at 10:07 AM
To: Kirsten Larson <kllarson@gmail.com>
Cc: Brad Whitmore <whitmore@stsci.edu>, Janice Lee <janice@ipac.caltech.edu>
Subject: 10 brightest and 10 faintest, < 5 myr clusters relative to the CO clouds in the disk regions.
 
Hi Kristen – I am still worried that we may be degrading the correlation between positions of associations and CO peaks by including  low S/N objects. Could you show an image and plot (for both 3351 and 1556) with ONLY the 10 brightest < 5 myr clusters relative to the CO clouds in the disk region.
 
Then try the same things for the 10 faintest (expect this one to be pretty random)
 
Then do the same for the oldest associations (expect these to be pretty random)
 
Sorry to keep pushing this but I am use to seeing the youngest, brightest clusters right on top of the Halpha, and since Halpha correlates well with CO, I expect the them to be right on top of the CO.
 
Cheers,
Brad
